Measurement of correlations between elliptic flow and mean transverse momentum in pp, p-Pb, and Pb-Pb collisions at the LHC

Measurements of the event-by-event correlation between elliptic flow ($v_2$) and the mean transverse momentum ($[p_{\rm T}]$) using the modified Pearson correlation coefficient $\rho(v_2^2,[p_{\rm T}])$ are reported in pp collisions at $\sqrt{s} = 13$ TeV, and in p-Pb and Pb-Pb collisions at a center-of-mass energy per nucleon pair $\sqrt{s_{\rm NN}} = 5.02$ TeV. This analysis is based on the full LHC Run 2 dataset recorded by ALICE and is performed for the first time in small collision systems with the ALICE detector. In Pb-Pb collisions, the $\rho(v_2^2,[p_{\rm T}])$ measurement shows a non-monotonic dependence on charged particle multiplicity ($N_{\rm ch}$); it first decreases and then increases with an increase in multiplicity. The decreasing trends of $\rho(v_2^2,[p_{\rm T}])$ with increasing multiplicity are also observed in p-Pb and pp collisions for the presented multiplicity range. All three systems show consistent values of $\rho(v_2^2,[p_{\rm T}])$ for $N_{\rm ch} \lesssim 80$. These measurements are also compared with theoretical model calculations, including PYTHIA, where no collectivity is generated, as well as AMPT and IP-Glasma + MUSIC + UrQMD, which produce collective effects in small systems. These comparisons offer unique insights into the origin of collectivity in small systems. They improve the understanding of the initial geometry, size, and their correlations. The comparison also allows an investigation of the role of initial momentum correlations predicted by the Color Glass Condensate framework. The new measurements could not be explained by current state-of-the-art models, offering insights into the initial stage of collisions in small systems and also imposing strong constraints on the existing theoretical models. This will significantly advance our understanding of the collective phenomena observed in small systems at the LHC.

==> observables.tex <==
\label{sec:ana-vnpt} 

These components are expressed as the formula of particle azimuthal angles and transverse momentum. All the particles used in the expressions are within $0.2 < \pt < 3.0~\mathrm{GeV}/c$.

\subsection{Covariance between \texorpdfstring{$v_2^2$}{v2} and \texorpdfstring{$[\pt]$}{pt}}

The covariance between $v_n^2$ and $[\pt]$ is expressed as
\begin{equation}
		\cov(v_2^2,[\pt])
= 
\Big\langle\frac{\displaystyle\sum_{i\in A,~j\in C }w_i w_j\cos(2\varphi_i-2\varphi_j)\sum_{k\in B} w_k^\mathrm{E}(p_{\mathrm{T},k}-\langle[\pt]\rangle)}{\displaystyle\sum_{i\in A,~j\in C}w_i w_j\sum_{k\in B} w_k^\mathrm{E}}
  \Big\rangle,
  \label{eq:covvnpt}
	\end{equation}
where the particles with indices $i$, $j$ are selected from subevents A ($\-0.8 < \eta < -0.4$) and C ($0.4 < \eta < 0.8$) and the particles with indices $k$ are selected from subevent B ($-0.4 < \eta < 0.4$). The subevent method ensures that non-flow is minimized in the azimuthal angle correlations and that there are no self-correlations between the flow and transverse momentum measurements. The  $w_i=w_{i}^\mathrm{A}w_i^\mathrm{E}$ ($w_j=w_{j}^\mathrm{A}w_j^\mathrm{E}$) is the weight for non-uniform detector acceptance correction ($w_{i(j)}^\mathrm{A}$) and $\pt$ dependent efficiency correction  ($w_{i(j)}^\mathrm{E}$), while the $w_k^\mathrm{E}$ is the weight for $\pt$ dependent efficiency correction only, described in Sec.~\ref{sec:cuts}. The $\varphi$ and $\pt$ are the azimuthal angle and transverse momentum of the corresponding particle. 

The $\langle[\pt]\rangle$ in Eq.~\ref{eq:covvnpt} is expressed as 
\begin{equation}
		\langle[\pt]\rangle = \Big\langle\frac{\displaystyle
			\sum_i w^{\mathrm{E}}_i p_{\mathrm{T}(i)}
		}{\displaystyle
			\sum_i w^{\mathrm{E}}_i
		}\Big\rangle,
\end{equation}
where $i$ loops over all the tracks in the kinematic region $|\eta| < 0.4, 0.2 < \pt < 3~\mathrm{GeV}/c$, and $w_i^\mathrm{E}$ is the weight for efficiency correction. 

\subsubsection{Variance of \texorpdfstring{$v_2^2$}{v2} and \texorpdfstring{$[p_\mathrm{T}]$}{pt}}
The square root of the variance of the $v_2^2$ is calculated as:
	\begin{equation}
 \begin{array}{cl}
		\sigma(v_2^2) &= 
		\sqrt{\var(v_2^2)} \\
	& = 
 \displaystyle\sqrt{
 \langle\langle\cos(2\varphi_1+2\varphi_2-2\varphi_3-2\varphi_4)\rangle\rangle_{|\Delta\eta| > 0.8} 
 -
 \langle\langle\cos(2\varphi_1-2\varphi_3)\rangle\rangle^2_{|\Delta\eta| > 0.8}}.
  \end{array}
  \label{eq:sigma}
	\end{equation}
The two-particle azimuthal correlation in Eq.~\ref{eq:sigma} could be expressed as:
\begin{equation}
\label{eq:cos22gap}
  \langle\langle \cos(2\varphi_1-2\varphi_2)\rangle\rangle_{|\Delta\eta| > 0.8}
= 
\Big\langle
\frac{\displaystyle\sum_{i,j}w_i w_j\cos(2\varphi_i-2\varphi_j)}{\displaystyle\sum_{i,j}w_i w_j}
\Big\rangle
,
\end{equation}
while $i$ loops over particles with $\eta < -0.4$, and $j$ loops over particles with $\eta > 0.4$.

Similarly the four-particle azimuthal correlation in Eq.~\ref{eq:sigma} is expressed as:
\begin{equation}
  \langle\langle \cos(2\varphi_1+2\varphi_2-2\varphi_3-2\varphi_4))\rangle\rangle_{|\Delta\eta| > 0.8}
= 
\Big\langle\frac{\displaystyle\sum_{i\neq j,k\neq l}w_i w_jw_k w_l\cos(2\varphi_i+2\varphi_j-2\varphi_k-2\varphi_l)}{\displaystyle\sum_{i\neq j,k\neq l}w_i w_j w_k w_l}
\Big\rangle,
\end{equation}
where $i,j$ loop over particles with $\eta < -0.4$ and $k,l$ loop overparticles with $\eta > 0.8$.

The variance of $[\pt]$ is calculated as:
\begin{equation}
	\langle\delta\pt^2\rangle = \Big\langle\frac{\displaystyle
		\sum_{i\neq j} w_{i}^\mathrm{E} w_{j}^\mathrm{E} (\pt^i - \langle[\pt]\rangle)(\pt^j - \langle[\pt]\rangle)
	}
	{\displaystyle
		\sum_{i\neq j} w_{i}^\mathrm{E} w_{j}^\mathrm{E}
	}\Big\rangle,
 \label{eq:deltapt}
\end{equation}
with $i$ and $j$ loop over particles within the kinematic region of $|\eta| < 0.4$.
